On the Power of Learning-Augmented Search Trees

We study learning-augmented binary search trees (BSTs) via Treaps with carefully designed priorities. The result is a simple search tree in which the depth of each item $x$ is determined by its predicted weight $w_x$. Specifically, each item $x$ is assigned a composite priority of $-\lfloor\log\log(1/w_x)\rfloor + U(0, 1)$ where $U(0, 1)$ is the uniform random variable. By choosing $w_x$ as the relative frequency of $x$, the resulting search trees achieve static optimality. This approach generalizes the recent learning-augmented BSTs [Lin-Luo-Woodruff ICML '22], which only work for Zipfian distributions, by extending them to arbitrary input distributions. Furthermore, we demonstrate that our method can be generalized to a B-Tree data structure using the B-Treap approach [Golovin ICALP '09]. Our search trees are also capable of leveraging localities in the access sequence through online self-reorganization, thereby achieving the working-set property. Additionally, they are robust to prediction errors and support dynamic operations, such as insertions, deletions, and prediction updates. We complement our analysis with an empirical study, demonstrating that our method outperforms prior work and classic data structures.

==> notused.tex <==

\subsection{Comparison with other Learned Data Structures}
We compared the performance of our learning-augmented Treaps with the learning-augmented skip-lists of \cite{fu2024learningaugmentedskiplists} on the AOL web query dataset (this paper also examined learning-augmented Treaps which we did not believe were a relevant comparison given that these data-structures are used for processing multi-dimensional data). We used some of the AOL data to pre-process the predicted frequencies for these data structures, and then used the remaining data to serve as the specific queries into these data structures. We saw \cref{fig:skiplists} that as the number of queries grew, the learning-augmented Treaps consistently performed better than the learning-augmented skip-lists, potentially because the Treaps are a more natural solution to finding queries that have some natural ordering in addition to implicit priority. % not sure about this theoretical justification
\begin{figure}[h!]
    \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{_images/zipf25err.png}
        \captionsetup{font=small} % Adjust caption size
        \caption{Mixture distribution, Zipfian has mixing weight 25\%.}
        \label{fig:25zipmix}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{_images/zipf50err.png}
        \captionsetup{font=small} % Adjust caption size
        \caption{Mixture distribution, Zipfian has mixing weight 50\%.}
        \label{fig:50zipmix}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{_images/zipf75err.png}
        \captionsetup{font=small} % Adjust caption size
        \caption{Mixture distribution, Zipfian has mixing weight 75\%.}
        \label{fig:75zipmix}
    \end{minipage}
       \centering
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{_images/uni25err.png}
        \captionsetup{font=small} % Adjust caption size
        \caption{Mixture distribution, uniform has mixing weight 25\%.}
        \label{fig:25unimix}
    \end{minipage}%
\end{figure}

\begin{figure}[h!]
     \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{_images/uni50err.png}
        \captionsetup{font=small} % Adjust caption size
        \caption{Mixture distribution, uniform has mixing weight 50\%.}
        \label{fig:50unimix}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{_images/uni75err.png}
        \captionsetup{font=small} % Adjust caption size
        \caption{Mixture distribution, uniform has mixing weight 75\%.}
        \label{fig:75unimix}
    \end{minipage}
    \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{_new_images/icml_kl5.png}
        \captionsetup{font=small} % Adjust caption size
        \caption{Differing KL-divergences on 5000 elements.}
        \label{fig:kl_div}
    \end{minipage}
        \begin{minipage}{0.32\textwidth}
        \centering
        \includegraphics[width=\linewidth]{_new_images/aol_v_skip_icml25.png}
        \captionsetup{font=small} % Adjust caption size
        \caption{Comparison of learned treaps vs. learned skip lists.}
        \label{fig:skiplists}
    \end{minipage}
\end{figure}

==> rebuttal <==
Reviewer HPYf：

I wonder whether there might be a misunderstanding on my side and authors can explain that. Looks to me that the statements of their theorem do not imply that their tree is never worse (even with very bad predictions) than a balanced tree built without any information about the input sequence. E.g., they seem to claim that their tree has O(log n) worst-case depth (line 310), but I do not see how does Thm 2.13 claim this.


A suggestion: you seem to call robustness what other papers in the area call smoothness or dependence on prediction error. Might be better to use the same terminology as other works.

Can you please explain the behavior of your data structures (both static and dynamic) with very bad predictions?

Looking at Theorem 2.13, if the real frequency of some element was a constant (0.1, let's say) and the predicted frequency was exp(-n), then the bound of Thm 2.13 on the access cost of your data structure would be mn while any balanced tree pays at most mlog(n). I.e., with very bad predictions, your tree seem to be much worse than a balanced tree built without any information about the input sequence, and is not "robust", in the sense commonly used e.g. in the survey of Mitzenmacher and Vassilvitskii which you cite in your paper.

their dynamic data structure requires a large branching factor (omega(log n)), i.e., it is far from a binary tree


Rebuttal:

Thanks for your comments! We will address your concern as follows.

**Robustness and Bad Predictions**

We use the word *robustness* to describe how the performance of our data structure degrades smoothly with respect to the prediction error - measured by KL divergence in the static setting and mean absolute error in the dynamic setting.

Using the robustness definition in [1][2] - i.e., the competitive ratio under the worst-case prediction - our data structure is $O(n)$-robust in the static setting (Proposition 2.3 in [2]). 

However, the data structure achieves $O(\log n)$-robustness if we ensure that each predicted score is at least $1/n^C$ for a large constant $C>0$. In practice, this can be achieved by modifying the predictor to guarantee it, for example, by taking a maximum of the predicted score and $1/n$. 

In the dynamic setting, assuming the predicted scores satisfy $\tilde{w}_{i,j}\geq 1/poly(n)$ as in Theorem 4.5, the data structure achieves $O(\log n)$-robustness.


**Worst-case Bound**
In Line 310, our intention was to illustrate that there exists a distribution under which the BSTs in Lin et al. have an $Omega(n)$ access cost, whereas our data structure achieves $O(\log n)$. We apologize for the unclear wording, which may have led to the misunderstanding that our method always guarantees $O(\log n)$ worst-case access cost. 

We will revise Line 310 as follows to clarify this point:

>However, it does not generally hold - there exists a distribution $p$ where the expected access cost for [3] is $\Omega(n)$, while our data structure achieves only $O(\log n)$ cost.


**Branching Factor**
The branching factor arises from B-treaps. If we want to construct a BST in the dynamic setting, the analysis proceeds in the same way, without involving the branching factor.


[1] Mitzenmacher, Michael, and Sergei Vassilvitskii. "Algorithms with predictions." Communications of the ACM 65.7 (2022): 33-35.
[2] Zeynali, Ali, Shahin Kamali, and Mohammad Hajiesmaili. "Robust Learning-Augmented Dictionaries." International Conference on Machine Learning. PMLR, 2024.
[3] Lin, Honghao, Tian Luo, and David Woodruff. "Learning augmented binary search trees." International Conference on Machine Learning. PMLR, 2022.

--------------------------------------------------------------------------------

Reviewer AYCV：

When discussing optimal static trees, the classic work of Knuth [Acta Informatica, 1971] may be cited. Additionally, two recent works on learning-augmented skip lists, which also explore topics such as static optimality, are Zeynali et al. [ICML 2024] and Fu et al. [ICLR 2025] (only the second one is mentioned briefly in the context of experiments).


1- The learning-augmented data structures presented in this paper achieve static optimality and the working-set property. However, these properties have already been established for classical data structures that do not rely on predictions, most notably splay trees. Could you clarify whether your data structures offer any notable theoretical advantages over splay trees?

2- What is the maximum depth of a node in your data structure? Is it possible that it gets linear depth under a highly skewed frequency distribution? In Line 096, you criticize the structure proposed by Lin et al. for having "super-logarithmic depth" in some cases, and this seems to be established in Theorem 2.14, where you demonstrate that assigning predicted frequencies directly as priorities (as in Lin et al.) results in linear depth and cost. How does this result compare to Proposition 2.2 in Zeynali et al. [ICML 2024]?

3- The structure proposed by Lin et al. [ICML 2022] appears to be deterministic, whereas your approach is randomized. Is there any known lower bound or negative result suggesting that deterministic data structures cannot achieve static optimality under prediction error?

Rebuttal:

Thanks for your thoughtful comments! We would like to begin by sincerely thanking you for pointing out the related work that we had overlooked. We will make sure to include proper citations in the updated version of the paper. Below, we address the three specific questions you raised:


1. Splay trees are conjectured to be dynamically optimal, which requires no prior knowledge. Therefore, it is very likely that no BST with/without learning-augmented can beat them in the theoretical bound. However, it is important to note that the runtime guarantees of splay trees are amortized. In particular, accessing a single item $x$ may still take linear time, which could be prohibitive in many scenarios. 

Furthermore, there are no "splay trees" in the B-tree area under the external-memory setting. This makes our approach more applicable in such settings.

We also observe from our experiment results that splay trees have a higher access cost across most datasets. In this way, our work contributes to the study and understanding of static and dynamic optimality in search trees and could serve as a useful step toward a better understanding of splay tree optimality.


2. When the frequency distribution is highly skewed, some items may have an exponentially small frequency. This can result in depths as large as $O(n)$. However, the data structure still achieves *static optimality*.

In contrast, for the data structure proposed by Lin et al., Theorem 2.14 shows a frequency distribution where the depth is $\Omega(n)$. This aligns with the consistency results of $\Omega(n/\log n)$ given in Proposition 2.2 of Zeyanali et al..


3. Exploring lower bounds for deterministic data structures in the learning-augmented setting is indeed an interesting and important direction. However, to the best of our knowledge, there are currently no established results in this area. We agree that this is a valuable question for future work.



--------------------------------------------------------------------------------



Reviewer tuW9：

In particular, I could not really understand the calculations in the section on the dynamic setting, because this section is quite technically involved, and not really written in an accessible way.

Please consider discussing and citing "Binary Search with Distributional Predictions" by Dinitz et al. (https://arxiv.org/abs/2411.16030) which appeared at NeurIPS 2024. That work seems quite relevant with the topic of this paper.

I do however feel that the paper could be written better. For example, I felt that the introduction was quite dense. In its present form, a lot of jargon is stated without having defined/described certain concepts. 

Correct me if I am wrong, but it seems like the guarantee in Theorem 2.8 of each node x having expected depth O(log(m/fx)) holds for any worst-case sequence of keys (even if they are not drawn iid from a distribution). It might be worth mentioning this somewhere after the Theorem.

Maybe I missed it, but I don't think there is clear mention of the fact that the optimal static cost (as established by Mehlhorn 1975) is on the order of the Shannon entropy of the distribution. You mention in Theorem 2.8 that the cost of your treap is O(\sigma fx log (m/fx)) matches the optimal static BST cost, but you haven't really stated anywhere what the static optimal BST cost is (unless I missed it) for the reader to really understand why this cost this optimal.


Could you please comment on the robustness properties of the treap constructed in Lin et al. 2022? I think the paper warrants a discussion/comment about this, either in the section where you do the robustness analysis of your treap, or at any other place where you cite Lin et al. 2022

I am likely failing to see something simple, but could you elaborate on why your 
O(log 1/wx) bound on the depth from Theorem 2.4 translates to an O(log n) bound? This would mean that wx>=1/n ---why is this true? You mention this in lines 309-310 in the section where you analyze alternate priority functions.

Rebuttal:

Thank you for your comments! We sincerely apologize for the various writing issues and will make every effort to improve them, particularly in the sections on the dynamic setting and the introduction. We will also cite the article you recommended and clearly state the static optimal BST cost to help readers better understand the context. Your writing suggestions are very helpful, and we truly appreciate you pointing them out. We address your question as follows.


1. The robustness in [Lin et al.] is defined as follows. If the frequency predictor satisfies $\frac{1}{\delta}f_i\leq \hat{f_i} \leq \delta f_i$ for some constant $\delta>0$, then the corresponding Treap with predicted score has an additive constant error compared to the optimal. 

    If we use the same definition, our data structure also achieves an additive constant error in access cost relative to the optimal. However, our notion of robustness provides a **stronger guarantee** -  even when the predicted frequency does not satisfy this assumption. In particular, we still obtain an upper bound on the access cost measured by the KL divergence. 



2. In Line 310, our intention was to illustrate that there exists a distribution under which the BSTs in Lin et al. have an $Omega(n)$ access cost, whereas our data structure achieves $O(\log n)$. We apologize for the unclear wording, which may have led to the misunderstanding that our method always guarantees $O(\log n)$ worst-case access cost. 

We will revise Line 310 as follows to clarify this point:

>However, it does not generally hold - there exists a distribution $p$ where the expected access cost for [3] is $\Omega(n)$, while our data structure achieves only $O(\log n)$ cost.


--------------------------------------------------------------------------------



Reviewer R8jP：

Typically, in the learning-augmented literature, the "robustness" guarantee is ideally asymptotically similar to the setting without predictions. The authors gave a robustness bound in terms of KL divergence between the true frequencies and predicted frequencies. I was hoping the authors can discuss and relate their bound with the setting without predictions.

While I can imagine how to get frequency predictions for the static setting, it is unclear how one can obtain the predictions needed for the dynamic setting to work well. I hope that the authors can point me to a discussion that I might have overlooked or mention what explanation they will add in their revision.

Clarification: In the proof plan on Page 4, the expected depth of x refers to the number of its ancestors, not just in S_t, right? If so, in the proof of Theorem 2.4 on Page 5, what about the ancestors of x outside of S_t? What am I misunderstanding?

I might have missed it but could you describe how the B-tree is being updated in the dynamic setting?


Rebuttal:

Thank you for your thoughtful comments! We address the questions and concerns as follows.

**Robustness**
If no prediction is available, we can naturally set the "predicted frequency" to be $1/n$. In this case, the access cost becomes $O(\log n)$. 


**Predictions for Dynamic Settings**
Thank you for highlighting this point! We will include a paragraph in the revision regarding the prediction of working-set scores.

> The working-set size (Definition 4.2) captures the temporal locality and diversity of user behavior around item $x$. Although it requires knowledge of future access items, it aligns conceptually with practices in recommendation systems, where temporal context is used to model user intent and predict relevance. For example, session-based recommendation often considers the diversity of items within a user's recent session [1]. In practice, we can approximate this score using causal proxies (e.g., past-only working-set size) or apply machine learning models to predict it based on observable access patterns.


**Clarification on Proof Plan**
The priority score of $x$ consists of the tier $\tau_x$, which is an integer, and $\delta_x \in (0,1)$. Consequently, all ancestors of the node $x$ must have tier less than or equal to $\tau_x$, and thus are part of the set $S_t$ for $t\leq \tau_x$. In other words, there are no ancestors of $x$ outside the sets $S_t$.

**B-tree Update**
At each time step, we first compute the working-set score of the current item, then remove the item from the B-tree, and finally re-insert the node into the B-tree with the updated score accordingly. Note that Treaps support insertions and deletions efficiently [Lemma 2.3].

[1] Wang, Shoujin, et al. "A survey on session-based recommender systems." ACM Computing Surveys (CSUR) 54.7 (2021): 1-38.


--------------------------------------------------------------------------------


